Machine learning and optimization-based approaches to duality in statistical physics

The notion of duality -- that a given physical system can have two different mathematical descriptions -- is a key idea in modern theoretical physics. Establishing a duality in lattice statistical mechanics models requires the construction of a dual Hamiltonian and a map from the original to the dual observables. By using simple neural networks to parameterize these maps and introducing a loss function that penalises the difference between correlation functions in original and dual models, we formulate the process of duality discovery as an optimization problem. We numerically solve this problem and show that our framework can rediscover the celebrated Kramers-Wannier duality for the 2d Ising model, reconstructing the known mapping of temperatures. We also discuss an alternative approach which uses known features of the mapping of topological lines to reduce the problem to optimizing the couplings in a dual Hamiltonian, and explore next-to-nearest neighbour deformations of the 2d Ising duality. We discuss future directions and prospects for discovering new dualities within this framework.

==> ml.tex <==
% \documentclass{article}
% \usepackage{graphicx} % Required for inserting images
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{mathtools}
% \usepackage{url}
% \usepackage{hyperref}

% %------Remove before submission ----------------------------------

% \usepackage[obeyFinal]{todonotes}
% \definecolor{prateekcolor}{RGB}{181,137,0}
% \definecolor{andreacolor}{RGB}{42,161,152}
% \definecolor{nabilcolor}{RGB}{242,200,152}
% \newcommand{\prateeknote}[2][]{\todo[color=prateekcolor,#1]{P: #2}}
% \newcommand{\andreanote}[2][]{\todo[color=andreacolor,#1]{A: #2}}
% \newcommand{\nabilnote}[2][]{\todo[color=nabilcolor,#1]{N: #2}}

% % margins


% \topmargin -0.06cm
% \oddsidemargin -0.04cm   % read Lamport p.163
% \evensidemargin -0.04cm  % same as oddsidemargin but for left-hand pages
% \textwidth 16.59cm
% \textheight 21.94cm
% %\pagestyle{empty}       % Uncomment if don't want page numbers
% \parskip 7.2pt           % sets spacing between paragraphs
% %\renewcommand{\baselinestretch}{1.5} 	% Uncomment for 1.5 spacing between lines
% \parindent 0pt	


% % nabil added shortcuts

% \newcommand{\be}{\begin{equation}}
% \newcommand{\ee}{\end{equation}}
% \newcommand{\bea}{\begin{eqnarray}}
% \newcommand{\eea}{\end{eqnarray}}
% \newcommand{\half}{\frac{1}{2}}
% \newcommand{\ehalf}{\frac{e}{2}}
% \newcommand{\ihalf}{\frac{i}{2}}
% \newcommand{\quart}{\frac{1}{4}}
% \newcommand{\G}{\Gamma}
% \renewcommand{\O}{\Omega}
% \renewcommand{\S}{\Sigma}
% \newcommand{\U}{\Upsilon}
% \renewcommand{\a}{\alpha}
% \renewcommand{\b}{\beta}
% \newcommand{\e}{\epsilon}
% \newcommand{\g}{\gamma}
% \renewcommand{\l}{\lambda}
% \newcommand{\s}{\sigma}
% \newcommand{\tB}{\tilde{B}}
% \newcommand{\tC}{\tilde{C}}
% \newcommand{\tR}{\tilde{R}}
% \newcommand{\tS}{\tilde{S}}
% \newcommand{\tL}{\tilde{L}}
% \newcommand{\ka}{\kappa}
% \newcommand{\derw}{{\bf\nabla}_w}
% \newcommand{\bA}{\overline{A}}
% \newcommand{\bC}{\overline{C}}



% \newcommand{\nn}{\nonumber\\}
% \newcommand{\bln}{\begin{align}}
% \newcommand{\eln}{\end{align}}
% \newcommand{\bst}{\begin{split}}
% \newcommand{\est}{\end{split}}
% \newcommand{\bi}{\begin{itemize}}
% \newcommand{\ei}{\end{itemize}}
% \newcommand{\ben}{\begin{enumerate}}
% \newcommand{\een}{\end{enumerate}}

% \def\AA{{\mathcal A}}
% \newcommand{\BB}{{\mathcal B}}


% \def\lad{L} %rob {l_{AdS}} changed notation because this is not the ads scale
% \def\lg{\lam_{GB}}
% \def\ns{N_{\sharp}}
% \def\tf{\tilde{f}}
% \def\w{\tilde{\om}}
% \def\q{\tilde{q}}

% \def\ov{\over}
% \def\le{\left}
% \def\ri{\right}
% \def\ha{{1\over 2}}

% \def\al{{\alpha}}
% \def\ket#1{|#1\rangle}
% \def\bra#1{\langle#1|}
% \def\vev#1{\langle#1\rangle}
% \def\det{{\rm det}}
% \def\tr{{\rm tr}}
% \def\Tr{{\rm Tr}}
% \def\NN{{\cal N}}
% \def\th{{\theta}}




% \def \ra {\rightarrow}


% \def\ep{{\epsilon}}
% \def\apr{{\alpha'}}
% \newcommand{\p}{\partial}
% \def\LL{{\cal L}}
% \def\TT{{\cal T}}
% \def\tir{{\tilde r}}

% \newcommand\ga{{\ensuremath{{\gamma}}}}
% \newcommand\Ga{{\ensuremath{{\Gamma}}}}


% \newcommand\sig{\sigma}
% \newcommand\Sig{\Sigma}
% \newcommand\lam{\lambda}
% \newcommand\Lam{\Lambda}
% \newcommand\om{\omega}
% \newcommand\Om{\Omega}
% \newcommand\vt{\vartheta}
% \newcommand\de{{\ensuremath{{\delta}}}}
% \newcommand\De{{\ensuremath{{\Delta}}}}
% \newcommand\vp{\varphi}

% \def\GeV{{\rm GeV}}
% \def\fm{{\rm fm}}
% \def\MeV{{\rm MeV}}
% \def\lam{{\lambda}}

% %\def\abs#1{\left| #1\right|}
% \def\bR{\mathop{\bf R}}
% %\def\bra#1{\left\langle #1\right|}
% \def\eeq{\end{equation}}
% \def\half{\frac{1}{2}}
% \def\Im{\mathop{\rm Im}}
% %\def\ket#1{\left| #1\right\rangle}
% \def\Re{\mathop{\rm Re}}
% \def\Tr{\mathop{\rm Tr}}
% \def\crbig{\\\noalign{\vspace {3mm}}}
% \newcommand{\HHH}{{\cal H}}

% \def\tg{{\tilde g}}
% \def\tR{{\tilde R}}
% \def\tnab{{\tilde \nabla}}
% \def\Rb{{[R^B]}}
% \def\htt{{\hat t}}
% \def\hx{{\hat x}}
% \def\hy{{\hat y}}
% \def\hz{{\hat z}}
% \def\hr{{\hat r}}
% \def\DD{{\cal D}}
% \newcommand{\reef}[1]{(\ref{#1})}
% \newcommand{\ssc}{\scriptscriptstyle}
% \newcommand{\eg}{{\it e.g.,}\ }
% \newcommand{\ie}{{\it i.e.,}\ }
% \newcommand{\comment}[1]{{\bf [[[#1]]]}}
% \newcommand{\X}[5]{X^{\ssc (#1)}_{\ #2 #3}{}^{#4 #5}}

% \newcommand\sA{{\ensuremath{{\mathcal A}}}}
% \newcommand\sB{{\ensuremath{{\mathcal B}}}}
% \newcommand\sC{{\ensuremath{{\mathcal C}}}}
% \newcommand\sD{{\ensuremath{{\mathcal D}}}}
% \newcommand\sF{{\ensuremath{{\mathcal F}}}}
% \newcommand\sI{{\ensuremath{{\mathcal I}}}}
% \newcommand\sG{{\ensuremath{{\mathcal G}}}}
% \newcommand\sH{{\ensuremath{{\mathcal H}}}}
% \newcommand\sL{{\ensuremath{{\mathcal L}}}}
% \newcommand\sM{{\ensuremath{{\mathcal M}}}}
% \newcommand\sN{{\ensuremath{{\mathcal N}}}}
% \newcommand\sO{{\ensuremath{{\mathcal O}}}}
% \newcommand\sV{{\mathcal V}}
% \newcommand\sJ{{\mathcal J}}
% \newcommand\sS{{\mathcal S}}
% \newcommand\sR{{\ensuremath{{\mathcal R}}}}

% \newcommand\tal{{\tilde \alpha}}
% \newcommand\ta{{\tilde a}}
% \newcommand\td{{\tilde d}}
% \newcommand\tA{{\tilde A}}
% \newcommand\tsD{{\tilde \sD}}
% \newcommand\tG{{\tilde G}}
% \newcommand\tow{{\tilde \om}}
% \newcommand\tk{{\tilde k}}
% \newcommand\tj{{\tilde j}}

% \newcommand\bc{{\bar c}}
% \newcommand\bb{{\bar b}}
% \newcommand\bw{{\bar w}}
% \newcommand\ba{{\overline a}}

% \newcommand\bpsi{{\bar \psi}}
% \newcommand\bPsi{{\overline \Psi}}
% \newcommand\bPhi{{\overline \Phi}}

% \newcommand\da{{\dagger}}
% \newcommand\nab{{\nabla}}
% \newcommand\Th{{\Theta}}
% \def\th{{\theta}}

% \newcommand\uz{{\underline{z}}}
% \newcommand\ut{{\underline({t}}}
% \newcommand\ur{{\underline{r}}}
% \newcommand\ui{{\underline{i}}}
% \newcommand\uj{{\underline{j}}}
% \newcommand\umu{{\underline{\mu}}}
% \newcommand\uM{{\underline{M}}}
% \newcommand\utau{{\underline{\tau}}}
% \newcommand\id{{\bf 1}}

% \newcommand\bg{{\overline{g}}}
% \newcommand\bG{{\overline{G}}}
% \newcommand\bsig{{\overline{\sig}}}
% \newcommand\bnab{{\overline{\nabla}}}
% \newcommand\bSig{{\overline{\Sig}}}
% \newcommand\bz{{\overline{z}}}
% \DeclareMathOperator*{\argmin}{arg\,min}
% \usepackage{algorithm}
% \usepackage{algpseudocode}

% \title{Duality}

% \begin{document}

% \maketitle
% \section{General neural network approach}

% \subsection{Motivation}
% The recent breakthroughs in machine learning and artificial intelligence are being employed in scientific advancements in physics, chemistry, and other life sciences~\cite{}.
% Such endeavours have the potential to extrapolate the existing results to the domain where sheer talent of the experts have failed from time to time. 
% In the same line of work, we propose to design an algorithm capable of reproducing the existing theoretical results in statistical duality. 
% Having such a capability will help us extend the algorithm to domains that have not previously been explored, potentially discovering new results. 
% In this section, we explore a general methodology to do so. 

\subsection{Methodology}
Given a system described by $\phi_i$, we propose a framework to algorithmically construct its dual. 
This framework exhibits two learnable components, $\tilde{H}$ and $G$, and a minimization objective function to match all possible moments (Eq. \ref{eq:}).
Mathematically, the framework aims to solve the following optimization problem:
\be
G^*, \tilde{H}^* = \argmin_{G, \tilde H} \mathcal{L}(\langle \mathbf{\Phi} \rangle_{H}, \langle \mathbf{\tilde\Phi} \rangle_{\tilde H})
\label{optim-framework}
\ee

The objective function is inspired by theoretical results~\cite{} requiring all the moments to be equal in the two frames.
We discuss the choice of such objective function in the subsequent section.

Specifically, we assume access to a sampler that generates $\phi$. 
The sampler configuration is defined through $H$ or $\tilde{H}$.
Given a well-defined objective function, we expect the loss to be minimum when the moments in the two frames match exactly, i.e., the loss goes to 0. 
However, this can happen in two scenarios - (a) $\tilde{H} = H$ and $G(\phi_i) = \phi_i$, i.e., the original frame is discovered, or (b) $\tilde{H} \neq H$ and $G(\phi_i) \neq \phi_i$, representing the dual system where moments perfectly match those of the original system.
We pictorially depict this framework in Fig.~\ref{fig:framework}.

\begin{figure*}[htp!]
    \centering
    \includegraphics[width=0.9\linewidth]{draft/images/framework.png}
    \caption{Neural network approach to constructing duality requires finding $\tilde{H}$ and $G$ that minimizes the loss defined by an appropriate moment-matching objective. }
    \label{fig:framework}
\end{figure*}

\paragraph{Kramers-Wannier (KW) Duality} We describe how the framework can be used to construct the KW duality for the 2D Ising model (Section~\ref{sec:kw}).

We assume access to a probabilistic sampler such as Markov Chain Monte Carlo (MCMC) that generates lattices for a given field configuration defined by $\beta \in \mathbf{R}$. 
We use " $\tilde{}$ '' to denote the parameters of the dual system. 
For example, $\beta$ and $\tilde{\beta}$ denote the field configurations for the original and the dual system respectively.
As specified in Section~\ref{sec:dualitybg}, the sampler generates lattices with probability distribution defined in Equation~\ref{isingH}.

We parameterize $G$ by a neural network with parameters $\mathbf{\theta}$, mapping a set of neighboring links to a scalar value.
Specifically, for a link defined by the lattice sites $i$ and $j$, we consider all the neighboring links as a vector input to $G_{\theta}$.
Figure~\ref{fig:linkMap} shows how we numbered the neighbouring links for vertical and horizontal links so that the resulting vector is rotationally invariant.

\begin{figure*}[htp!]
    \centering
    \includegraphics[width=0.5\linewidth]{draft/images/link-map.png}
    \caption{For KW duality, we parametrize $G$ as a neural network that takes neighboring links as its input. These links are provided as a vector where the numbers denote their position in the input vector. We use a numbering system that is rotationally invariant, a requirement for a symmetric system.}
    \label{fig:linkMap}
\end{figure*}


We resort to gradient descent approach for solving the above optimization problem.
Thus, our strategy to obtain $\theta^*$ and $\tilde{\beta}^*$ is to obtain gradients from the loss function $\mathcal{L}$ and apply them iteratively until the loss function is minimized.
\be
\theta \leftarrow \theta - \frac{\partial \mathcal{L}(\langle \mathbf{\Phi} \rangle_{H}, \langle \mathbf{\tilde\Phi} \rangle_{\tilde H})}{\partial \theta} \text{  ; } 
\tilde \beta \leftarrow \tilde \beta - \frac{\partial \mathcal{L}(\langle \mathbf{\Phi} \rangle_{H}, \langle \mathbf{\tilde\Phi} \rangle_{\tilde H})}{\partial \tilde \beta}
\label{gradUpdates}
\ee

We obtain gradients for $\theta$ using backpropagation through neural networks. 
However, since we can't backpropagate through a stochastic sampler, we derive the gradients $\frac{\partial \mathcal{L}(\langle \mathbf{\Phi} \rangle_{H}, \langle \mathbf{\tilde\Phi} \rangle_{\tilde H})}{\partial \tilde \beta}$ as in Appendix~\ref{app:gradBeta} and apply them at every iteration. 

\paragraph{Beyond KW Duality}

Extending the framework beyond the KW duality, we define a generalized Hamiltonian as a sum over terms, each of which contains one or more links, i.e., 
\be
\sH = -\sum_n \beta_n C_n(\sig) = -\sum_{n} \beta_n \prod_{\vev{ij} \in L_n} t_{\vev{ij}} \sig_i \sig_j \label{monomialdef} 
\ee
where each of the $L_n$ is a set of links. For $n=1$ and $C(\sigma) = \sum_{\langle ij \rangle} \sigma_i \sigma_j$, we obtain the previous case. 

Thus, instead of a single scalar $\beta$, we optimize for a vector $\mathbf{B} = (\beta_0, \beta_1, \cdot)$.
As a result, our gradient updates correspond to the vector $\mathbf{B}$ instead of individual scalar $\beta$s. 
We show the derivation in Appendix~\ref{app:gradBeta}. 

\subsection{Experiments}

In this section, we conduct experiments to establish KW duality using our framework.
We define an appropriate objective function for matching all sets of moments. 
Further, we define the neural network architecture. 
Finally, we empirically illustrate the construction of duality using the plots showing the progression of learning methods.

\paragraph{Objective function}
\begin{figure*}[htp!]
    \centering
    \includegraphics[width=\linewidth]{draft/images/loss_landscape_feats_N=8_beta_target=0.3.png}
    \caption{We visualize the loss landscapes for $\beta=0.3$ as a function of the number of features. Each column represents one, up to 7, or 13 features included in the loss function. (Top-row) $\beta=\tilde\beta$ while the mapping of +1 and -1 are varied, (Middle-row) Mapping of +1 is kept optimal while $\beta$ and mapping of -1 is varied, (Bottom-row) Mapping of -1 is kept optimal while $\beta$ and mapping of +1 is varied. <ADD OBSERVATION> }
    \label{fig:linkMap}
\end{figure*}


@Andrea and NI --- 
Description of the moments needed to match goes here.

Kernel?

Simple features?

\begin{figure*}[htp!]
    \centering
    \includegraphics[width=\linewidth]{draft/images/loss_landscape_kernel_N=8_beta_target=0.3.png}
    \caption{We visualize the loss landscapes for $\beta=0.3$ as a function of the kernel loss. Each column represents a slice of $\beta$, mapping of +1, and mapping of -1. <ADD OBSERVATION> {\bf Note at the moment this does not seem consistent with earlier work.}}
    \label{fig:linkMap}
\end{figure*}

\paragraph{Neural Network architecture, $G_{\theta}$} 
We considered a simplistic neural network architecture. 
Given a featurized vector $\mathbf{f}_{ij} \in \mathcal{R}^7$, we consider a neural network formed by $\theta_1 \in \mathcal{R}^7$, and scalars $\theta_2$ and $\theta_3$.
We opt for hard attention using Gumbel-Softmax~\cite{} so that only a few features are utilized in the prediction task.
This constraint can also be enforced by augmenting the loss function with entropy minimization term over $\theta_1$.
In this work, we chose to use the Gumbel-Softmax trick commonly used in the deep learning literature to sample discrete categorical variables in a differentiable manner. 

Thus, the mapping is defined by, 
\be
G_{\theta} (\mathbf{f}_{ij}) = \theta_2 \cdot \text{Gumbel-Softmax}(\theta_1)^{T}\mathbf{f}_{ij} + \theta_3
\label{eq:nnet}
\ee

We ran an ablation to check what would happen if we were not to use $\text{Gumbel-Softmax}$. 
We observe that a mapping of the form $G_{\theta} (\mathbf{f}_{ij}) = \theta_2 \cdot \theta_1^{T}\mathbf{f}_{ij} + \theta_3$ could work in some cases.
Specifically, we see that while most of our training runs didn't yield a sensible outcome, some combination of features can yield an original frame or dual frame. 
We show some of them in Figure~\ref{fig:no-gumbel-training}.


\paragraph{KW Duality}
In Figure~\ref{fig:beta-betaTilde}, we show the result of deploying the above machinery on different target values of $\beta$.
Specifically, for each value of the target $\beta$, we ran a total of 10 optimizations, five from each of the two initializations of $\beta$, i.e., $\beta_0=0.2$ and $\beta_0=0.4$. 
Due to the randomness involved in sampling, each seed is expected to be an independent run.
Note that the method doesn't work for values of $\beta$ after the phase transition.
We think it's because [@Andrea \& NI].

\begin{figure*}[htp!]
    \centering
    \includegraphics[width=0.8\linewidth]{draft/images/beta-betaTilde.png}
    \caption{Final $\tilde\beta$ as found by the deep learning framework closely matches that of the theoretical results. We expected the loss to be minimum along exactly two fronts, i.e, original frame $\beta = \tilde\beta$ and the dual frame along the lines $\sinh(2\beta)\sinh(2\tilde\beta) = 1$. }
    \label{fig:beta-betaTilde}
\end{figure*}

Further, we observe that the initialization of $\beta$ has an impact on the frame that is discovered.
We find that $\beta_0=0.4$ almost always drifted away from the original frame as indicated by the absence of green points on the $\beta = -\tilde\beta$ line. 
Note for $\beta=0.35$, we see a suboptimal run resulting in the final $\beta$ far away from the dual or original frame.
Figure~\ref{fig:trainingPlots} shows three runs from $\beta=0.35$ illustrating how the training progresses under different scenarios. 
For the seeds where either dual or original frame is recovered, the loss goes to 0. 
Further, we track the entropy of $\text{Gumbel-Softmax}(\theta_1)$ to assess how the algorithm is weighing each feature. 
A value of 0 corresponds to a strong preference for one out of seven dimensions.
We also show the training progress of the seed that yielded a non-optimal $\beta$ that ends at a higher loss than the rest. 

\begin{figure*}[htp!]
    \centering
    \includegraphics[width=0.8\linewidth]{draft/images/loss_trajectory.png}
    \caption{Training progress for handpicked runs from $\beta=0.35$ to showcase the trajectory of various metrics. 
    We show exponentially smoothed moving average of the following metrics: (A) Loss, (B) $\beta$, (C) Mapping, (D) Entropy of $\text{Gumbel-Softmax}(\theta_1)$}
    \label{fig:loss_trajectory}
\end{figure*}

Finally, we look at the dimension of $\mathbf{f}_{ij}$ that was selected to define the mapping.
Figure~\ref{fig:selected_dim} shows the distribution of the selected link.
$6$ corresponds to the original link, while $2$ and $5$ corresponds to the dual frame. 
We also observed a small number of runs that got stuck in local optima, resulting in the selection of $0$ or $4$. 

\begin{figure*}[htp!]
    \centering
    \includegraphics[width=0.8\linewidth]{draft/images/selected_dim.png}
    \caption{Corresponding to Figure~\ref{fig:beta-betaTilde}, we plot the frequency with which the dimension of the feature vector $\mathbf{f}_{ij}$ was selected. Note that $6$ corresponds to the link itself corresponding to the discovery of the original frame, $2$ and $5$ are symmetric and results in the dual frame, and the selection of $0$ and $4$ corresponds to the failed runs, which might be perhaps because of getting lost in the landscape and never getting out of the sub-optimal areas. }
    \label{fig:selected_dim}
\end{figure*}


\subsection{Discussion}

\begin{itemize}
\item Extending beyond the 13 features
\item Kernel design for the loss function
\item using Sparse attention to facilitate attention on more than two links in the mapping
\item stabilizing learning in a general case
\end{itemize}


% \appendix

% \section{Neural Network Training}
% Our models are all implemented in PyTorch~\cite{paszke2017automatic}. 
% We used the Adam~\cite{kingma2014adam} optimizer with the learning rate of $0.01$ for both $\beta$ and $\theta$.
% Moreover, we used the early stopping criterion to stop the training if the loss didn’t improve over 200 epochs. 
% We ran the sampler in each experiment to generate 1000 samples for the lattice. 
% We ran the training for a maximum of 25000 epochs, and our runs took about 1-3 hours each. 


% \section{Loss landscape after phase transition}

% \begin{figure*}[htp!]
%     \centering
%     \includegraphics[width=\linewidth]{draft/images/loss_landscape_feats_N=12.png}
%     \caption{The formation of valleys beyond the phase transition creates a problem where the minimum loss appears to be in a valley, resulting in a continual drift along the valley once low loss values are reached. }
%     \label{fig:selected_dim}
% \end{figure*}

% \begin{algorithm}
% \caption{Gradient-Based Optimization for Lattice Sampling}
% \begin{algorithmic}[1]
%     \State \textbf{Inputs:} $\beta$, $\eta$ (learning rate), $N$ (number of samples)
%     \State \textbf{Initialize:} $\beta_0 \in \mathbb{R}$, $\theta \in \mathbb{R}^d$
%     \For{each epoch $t = 1, 2, \dots, T$}
%         \State Draw $N$ samples $\{\phi_i\}_{i=1}^{N} \sim p(\phi | \beta)$
%         \State Draw $N$ samples $\{\phi_i'\}_{i=1}^{N} \sim p(\phi | \beta')$ where $\beta' \neq \beta$
%         \State Compute the loss $\mathcal{L} = \frac{1}{N} \sum_{i=1}^{N} \mathcal{L}(\phi_i, G_{\theta}(\phi_i'))$
%         \State Compute the gradients $\nabla_{\beta} \mathcal{L}$ and $\nabla_{\theta} \mathcal{L}$
%         \State Update the parameters:
%         \begin{align*}
%             \beta_{t+1} &\gets \beta_t - \eta \nabla_{\beta} \mathcal{L} \\
%             \theta_{t+1} &\gets \theta_t - \eta \nabla_{\theta} \mathcal{L}
%         \end{align*}
%         \If{$\mathcal{L}$ has not improved for the last $X$ epochs}
%             \State \textbf{Stop the optimization}
%         \EndIf
%     \EndFor
% \end{algorithmic}
% \end{algorithm}

% \bibliographystyle{utphys}
% \bibliography{all}
% \end{document}

